Low Latency Transformer Inference on FPGAs for Physics Applications with hls4ml

This study presents an efficient implementation of transformer architectures in Field-Programmable Gate Arrays(FPGAs) using hls4ml. We demonstrate the strategy for implementing the multi-head attention, softmax, and normalization layer and evaluate three distinct models. Their deployment on VU13P FPGA chip achieved latency less than 2us, demonstrating the potential for real-time applications. HLS4ML compatibility with any TensorFlow-built transformer model further enhances the scalability and applicability of this work. Index Terms: FPGAs, machine learning, transformers, high energy physics, LIGO

==> outlook.tex <==
\section{Outlook}
\label{sec:outlook}

FPGAs have been traditionally been used for various specialized tasks.
Their low power consumption and extremely fast processing make them particularly suited for applications across industry and high energy physics.
Their advantages, however, are not exclusive to these domains and can be leveraged for many other high-performance computing tasks.


==> quantization.tex <==
\section{Quantization}
\label{sec:quantization}

Quantization-Aware Training (QAT) in essence is about training the model under the same constraints it will experience during its inference in a quantized state. This method is known to yield models that are more robust and resilient to the quantization errors because the model is aware of these quantization intricacies during its training phase. As a result, QAT often leads to better model accuracy post-quantization compared to PTQ, especially for lower bit-widths.

